Linguistic Structure Induction from Language Models

Linear sequences of words are implicitly represented in our brains by hierarchical structures that organize the composition of words in sentences. Linguists formalize different frameworks to model this hierarchy; two of the most common syntactic frameworks are Constituency and Dependency. Constituency represents sentences as nested groups of phrases, while dependency represents a sentence by assigning relations between its words. Recently, the pursuit of intelligent machines has produced Language Models (LMs) capable of solving many language tasks with a human-level performance. Many studies now question whether LMs implicitly represent syntactic hierarchies. This thesis focuses on producing constituency and dependency structures from LMs in an unsupervised setting. I review the critical methods in this field and highlight a line of work that utilizes a numerical representation for binary constituency trees (Syntactic Distance). I present a detailed study on StructFormer (SF) (Shen et al., 2021), which retrofits a transformer encoder architecture with a parser network to produce constituency and dependency structures. I present six experiments to analyze and address this field's challenges; experiments include investigating the effect of repositioning the parser network within the SF architecture, evaluating subword-based induced trees, and benchmarking the models developed in the thesis experiments on linguistic tasks. Models benchmarking is performed by participating in the BabyLM challenge, published at CoNLL 2023 (Momen et al., 2023). The results of this thesis encourage further development in the direction of retrofitting transformer-based models to induce syntactic structures, supported by the acceptable performance of SF in different experimental settings and the observed limitations that require innovative solutions to advance the state of syntactic structure induction.

==> cd.tex <==
\chapter*{}
\thispagestyle{empty}

\begin{center}
  \vspace{-3cm}
  \fbox{\parbox[c][12cm][c]{12cm}{\centering Hier die Hülle\\[1cm]mit der CD/DVD einkleben}}
\end{center}

\vfill

\textbf{Diese CD enthält:}
\begin{itemize}
 \item eine \emph{pdf}-Version der vorliegenden \thesistype{}
 \item die \LaTeX- und Grafik-Quelldateien der vorliegenden \thesistype{} samt aller verwendeten Skripte
 \item \textbf{[anpassen]} die Quelldateien der im Rahmen der \thesistype{} erstellten Software XYZ
 \item \textbf{[anpassen]} den zur Auswertung verwendeten Datensatz
 \item die Websites der verwendeten Internetquellen
\end{itemize}

